Acceleration Algorithms in GNNs: A Survey

Graph Neural Networks (GNNs) have demonstrated effectiveness in various graph-based tasks. However, their inefficiency in training and inference presents challenges for scaling up to real-world and large-scale graph applications. To address the critical challenges, a range of algorithms have been proposed to accelerate training and inference of GNNs, attracting increasing attention from the research community. In this paper, we present a systematic review of acceleration algorithms in GNNs, which can be categorized into three main topics based on their purpose: training acceleration, inference acceleration, and execution acceleration. Specifically, we summarize and categorize the existing approaches for each main topic, and provide detailed characterizations of the approaches within each category. Additionally, we review several libraries related to acceleration algorithms in GNNs and discuss our Scalable Graph Learning (SGL) library. Finally, we propose promising directions for future research. A complete summary is presented in our GitHub repository: https://github.com/PKU-DAIR/SGL/blob/main/Awsome-GNN-Acceleration.md.

==> Figure/T1.tex <==
\definecolor{mylightred}{RGB}{255,192,203}
\definecolor{mylightorange}{RGB}{255,218,185}
\tikzset{
  FARROW/.style={arrows={-{Latex[length=1.25mm, width=1.mm]}}, }, %thick
  U/.style = {circle, draw=melon!400, fill=melon, minimum width=1.4em, align=center, inner sep=0, outer sep=0},
  I/.style = {circle, draw=tea_green!400, fill=tea_green, minimum width=1.4em, align=center, inner sep=0, outer sep=0},
    cate0/.style = {rectangle, draw, minimum width=4cm, minimum height=1cm, align=left, rounded corners=3,draw=mylightred}, 
    cate1/.style = {rectangle, draw, minimum width=2cm, minimum height=0.8cm, align=left, rounded corners=3,draw=mylightred}, %fill=Madang!82,
    cate2/.style = {rectangle, draw, text width=15cm, minimum height=0.8cm, align=left, rounded corners=3,draw=mylightred,fill=mylightorange}, 
    cate3/.style = {rectangle, draw, minimum width=3.7cm, minimum height=0.8cm, align=left, rounded corners=3,draw=mylightred},
   %fill=Madang!82,
  encoder/.style = {rectangle, fill=Madang!82, minimum width=10em, minimum height=3em, align=center, rounded corners=3},
}

\begin{figure*}
    \centering
    \resizebox{0.94\linewidth}{!}
    {\begin{tikzpicture}
    \node [cate0, distance=0cm, yshift=0cm, align=left,rotate=90,font=\large] (n1) at (0, 0) {\textbf{Acceleration Algorithms in GNNs}};
    \node [cate1, right of=n1, node distance=3cm, yshift=4cm] (n11) 
    {\textbf{GNN Training}}; 
    \node [cate1, below=4cm of n11.west, anchor=west] (n12) 
    {\textbf{GNN Inference}};  
    \node [cate1, below=4cm of n12.west, node distance=5cm, anchor=west] (n13) {\textbf{GNN Execution}};
    \draw[] (n1.south) -- (n11.west);
    \draw[] (n1.south) -- (n12.west)
    \draw[] (n1.south) -- (n13.west);
    \node [cate3, right of=n11, node distance=4cm, yshift=3cm,] (n111) {\textbf{Graph Sampling}};
    \node [cate3, below=3.5cm of n111.west, anchor=west] (n112) {\textbf{GNN Simplification}};
    \draw[] (n11.east) -- (n111.west);
    \draw[] (n11.east) -- (n112.west);
    \node [cate2, right of=n111, node distance=11cm, yshift=2cm] (n1111) 
    {\textbf{Node-wise Sampling:} 
        GraphSage \cite{GraphSage},
        PinSage \cite{PinSage},
        VR-GCN  \cite{VR-GCN},
        BNS \cite{BNS},
        GNN-BS \cite{GNN-BS},
        PASS \cite{PASS}
        ANS-GT \cite{ANS-GT}
    };
    \node [cate2, below=1.3cm of n1111.west, anchor=west] (n1112) 
    {\textbf{Layer-wise Sampling:}
        FastGCN \cite{FastGCN},
        AS-GCN \cite{ASGCN},
        LADIES \cite{LADIES},
        GRAPES \cite{GRAPES}
    };
    \node [cate2, below=1.3cm of n1112.west, anchor=west] (n1113) 
    {\textbf{Graph-wise Sampling:}
        Cluster-GCN \cite{ClusterGCN},
        GraphSAINT \cite{GraphSAINT},
        LGCL \cite{LGCL},
        SHADOW-GNN  \cite{SHADOW-GNN},
        GNNAutoScale \cite{GNNAutoScale},
        MVS-GNN \cite{MVS-GNN},
        RWT\cite{RWT},
        LMC \cite{LMC}
    };
    \draw[] (n111.east) -- (n1111.west);
    \draw[] (n111.east) -- (n1112.west);
    \draw[] (n111.east) -- (n1113.west);
    %right of=n111, node distance=8cm, yshift=2cm
    \node [cate2, below=1.7cm of n1113.west, anchor=west] (n1121) 
    {\textbf{Simple model without attention:} 
        SGC \cite{SGC},
        S\textsuperscript{2}GC \cite{S2GC},
        SIGN \cite{SIGN},
        GBP \cite{GBP},
        PPRGo \cite{PPRGo},
        NDLS \cite{NDLS},
        %Lasagne \cite{Lasagne},
        AGP \cite{AGP},
        NAFS \cite{NAFS},
        APPNP \cite{APPNP},
        C\&S \cite{C&S}
    };
    \node [cate2, below=1.7cm of n1121.west, anchor=west] (n1122) 
    {\textbf{Difficult model with attention:}
        SAGN \cite{SAGN},
        GA-MLP \cite{GAMLP},
        PaSca \cite{pAScA},
        NIGCN \cite{NIGCN},
        SCARA \cite{SCARA},
        Grand+ \cite{GRAND+}
    };
    \draw[] (n112.east) -- (n1121.west);
    \draw[] (n112.east) -- (n1122.west);
    \node [cate3, below=2.55cm of n112.west, anchor=west] (n121) {\textbf{Knowledge Distillation}};
    \node [cate3, below=2cm of n121.west, anchor=west] (n122) {\textbf{GNN Quantization}};
    \node [cate3, below=1.3cm of n122.west, anchor=west] (n123) {\textbf{GNN Pruning}};
    \draw[] (n12.east) -- (n121.west);
    \draw[] (n12.east) -- (n122.west);
    \draw[] (n12.east) -- (n123.west);
    %right of=n111, node distance=8cm, yshift=2cm
    \node [cate2, below=1.3cm of n1122.west, anchor=west] (n1211) 
    {\textbf{GNN-to-GNN:} 
        LSP \cite{LSP},
        TinyGNN \cite{TinyGNN},
        G-CRD  \cite{G-CRD},
        GFKD \cite{GFKD},
        KDEP \cite{KDEP},
        GKD \cite{GKD}
        
    };
    \node [cate2, below=1.3cm of n1211.west, anchor=west] (n1212) 
    {\textbf{GNN-to-MLP:}
        Graph-MLP \cite{Graph-MLP},
        GLNN \cite{GLNN},
        CPF \cite{CPF},
        NOSMOG \cite{NOSMOG},
        VQGraph \cite{VQGraph},
        KRD \cite{KRD},
        P\&D \cite{P&D}
    };
    \draw[] (n121.east) -- (n1211.west);
    \draw[] (n121.east) -- (n1212.west);
    \node [cate2, below=1.45cm of n1212.west, anchor=west] (n1221) 
    {LPGNAS \cite{LPGNAS},
     Degree-Quant \cite{Degree-Quant},
     SGQuant \cite{SGQuant},
     VQ-GNN \cite{VQ-GNN},
     A\textsuperscript{2}Q \cite{A2Q},
     EPQuant \cite{EPQuant},
     QLR \cite{QLR},
     %DBQ \cite{DBQ},
     \cite{Haar}
     %,MEGA\cite{MEGA}
    };
    \draw[] (n122.east) -- (n1221.west);
    \node [cate2, below=1.3cm of n1221.west, anchor=west] (n1231) 
    {\cite{Channel-Pruning},
     UGS \cite{UGS},
     ICPG\cite{Inductive},
     \cite{GEB},
     DLTH \cite{DLTH},
     \cite{improved-UGS},
     Snowflake \cite{Snowflake}
    };
    \draw[] (n123.east) -- (n1231.west);
    \node [cate3, below=1.2cm of n123.west, anchor=west] (n131) 
    {\textbf{GNN Binarization}};
    \node [cate3, below=1.4cm of n131.west, anchor=west] (n132) 
    {\textbf{Graph Condensation}};
    \draw[] (n13.east) -- (n131.west);
    \draw[] (n13.east) -- (n132.west);
    \node [cate2, below=1.2cm of n1231.west, anchor=west] (n1311) 
    {Bi-GCN \cite{Bi-GCN},
     BGN \cite{BGN},
     \cite{BinaryGNN},
     Meta-Aggregator \cite{Meta-Aggregator},
     BitGNN \cite{BitGNN}
    };
    \draw[] (n131.east) -- (n1311.west);
    \node [cate2, below=1.1cm of n1311.west, anchor=west] (n1321) 
    {
     \textbf{Node classification:} 
     GCond \cite{GCOND},
     SFGC \cite{SFGC},
     MCond \cite{MCond},
     GCDM \cite{GCDM},
     GCEM \cite{GCEM},
     GC-SNTK \cite{GC-SNTK}
    };
    \draw[] (n132.east) -- (n1321.west);
    \node [cate2, below=1cm of n1321.west, anchor=west] (n1321) 
    {
     \textbf{Graph classification:}
     DosCond \cite{DosCond},
     KIDD \cite{KIDD}
    };
    \draw[] (n132.east) -- (n1321.west);
    \end{tikzpicture}}
    \caption
    {
        {Taxonomy of GNN acceleration algorithms. We comprehensively introduce GNNs training acceleration in Section 3, GNNs inference acceleration in Section 4 and GNNs execution acceleration in Section 5, followed by our discussions of related libraries in Section 6 and future research directions in Section 7.}
    }
    \label{fig:user-item-summ-fig}
\end{figure*}



